Dignit\'e - DIGital Network Information & Traces Extraction

Web-based criminality like counterfeiting uses web applications which are hosted on web servers. Those servers contain a lot of information which can be used to identify the owner and other connected persons like hosters, shipping partners, money mules and more. These pieces of information reveal insights on the owner or provider of a fraud website, thus we can call them traces. These traces can then be used by the police, law enforcement authorities or the legal representatives of the victim. In our project 2 we had identified a vast range of possible traces. We had also considered their information content and existing limitations. During our Bachelor thesis, we have selected several traces and started the implementation of the API with its underlying library. After the successful implementation of the selected traces, we have created a graphical user interface to allow the use of our solution without using a command-line interface. To do so, we have learned to use the Scala Programming Language and its integration with Java code. The graphical user interface of our example application is built using Scala Swing, the Scala adoption of the Swing Framework. The test cases are defined using ScalaTest with FlatSpec and Matchers and executed using the JUnit Runner.

==> vorspann/titelseite_ohne_bild.tex <==
% !TeX encoding = UTF-8
%
% Project documentation template
% ===========================================================================
% This is part of the document "Project documentation template".
% Authors: brd3, kaa1
%

\begin{titlepage}


% BFH-Logo absolute placed at (28,12) on A4 
% Actually not a realy satisfactory solution but working.
%---------------------------------------------------------------------------
\setlength{\unitlength}{1mm}
\begin{textblock}{20}[0,0](28,12)
	\includegraphics[scale=1.0]{bilder/BFH_Logo_B.png}
\end{textblock}
\color{black}

% Institution / Titel / Untertitel / Autoren / Experten:
%---------------------------------------------------------------------------
\begin{flushleft}

\vspace*{21mm}

\fontsize{26pt}{40pt}\selectfont 
\titel 				\\							% Titel aus der Datei vorspann/titel.tex lesen
\vspace{2mm}

\fontsize{16pt}{24pt}\selectfont\vspace{0.3em}
\untertitel 				\\							% Untertitel aus der Datei vorspann/titel.tex lesen
\vspace{5mm}

\fontsize{10pt}{12pt}\selectfont
\textbf{Bachelor Thesis} \\									% eingeben
\vspace{7mm}

% Abstract (eingeben):
%---------------------------------------------------------------------------
\begin{textblock}{150}(28,100)
\fontsize{10pt}{12pt}\selectfont
\end{textblock}

\begin{textblock}{150}(28,225)
\fontsize{10pt}{17pt}\selectfont
\begin{tabbing}
xxxxxxxxxxxxxxx\=xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx \kill
Branch:	\> Computer Science	\\			% Namen eingeben
Authors:		\> Thomas Ender, Patrick Vananti	\\					% Namen eingeben
Advisor:	\> Claude Fuhrer (Olivier Biberstein)		\\					% Namen eingeben
Expert:		\> Dr. Joachim Wolfgang Kaltz				\\					% Namen eingeben
Date:			\> \versiondate					\\		% aus Datei vorspann/version.tex lesen
\end{tabbing}

\end{textblock}
\end{flushleft}

\begin{textblock}{150}(28,280)
\noindent 
\color{bfhgrey}\fontsize{9pt}{10pt}\selectfont
Berner Fachhochschule | Haute école spécialisée bernoise | Bern University of Applied Sciences
\color{black}\selectfont
\end{textblock}


\end{titlepage}

%
% ===========================================================================
% EOF
%

